Rethinking Fair Representation Learning for Performance-Sensitive Tasks

We investigate the prominent class of fair representation learning methods for bias mitigation. Using causal reasoning to define and formalise different sources of dataset bias, we reveal important implicit assumptions inherent to these methods. We prove fundamental limitations on fair representation learning when evaluation data is drawn from the same distribution as training data and run experiments across a range of medical modalities to examine the performance of fair representation learning under distribution shifts. Our results explain apparent contradictions in the existing literature and reveal how rarely considered causal and statistical aspects of the underlying data affect the validity of fair representation learning. We raise doubts about current evaluation practices and the applicability of fair representation learning methods in performance-sensitive settings. We argue that fine-grained analysis of dataset biases should play a key role in the field moving forward.

==> biblatex.tex <==
% An actually decent referencing style. C. Jones 2025.
\PassOptionsToPackage{
    style=authoryear, % Harvard/APA ish
    backend=bibtex, 
    natbib=true, % use \citep, \citet
    backref=true, % include links from bibliography back to text
    maxbibnames=99, maxcitenames=2, % show all names in bibliography, but up to 2 in-text
    uniquelist=false, uniquename=false, % don't try to disambiguate name clashes in-text
    date=year, % don't include months in bibliography
    dashed=false, giveninits=true,
    sorting=nyt, sortcites=false, 
    isbn=false,doi=false,url=false,eprint=false, % don't include links (we will hyperlink the titles instead)
}{biblatex}
\RequirePackage{biblatex}

\DeclareNameAlias{sortname}{family-given} % Lastname, Firstname in reference list

% Simplify references by removing superfluous fields.
% remove publisher for everything other than books.
\AtEveryBibitem{
 \clearlist{address}
 \clearfield{date}
 \clearfield{eprint}
 \clearfield{isbn}
 \clearfield{issn}
 \clearlist{location}
 \clearfield{month}
 \clearfield{series}
 \clearname{editor}
 
 \ifentrytype{book}{}{
   \clearlist{publisher}
 }
}

% use '&' instead of 'and' for consistency with natbib
\renewcommand*{\finalnamedelim}{%
    \ifnumgreater{\value{liststop}}{2}{\finalandcomma}{}%
    \addspace\&\space}%

% backref format
\DefineBibliographyStrings{english}{backrefpage={cited on p.},backrefpages={cited on pp.}} 

% \renewcommand*{\bibfont}{\normalfont\small} % make bibliography use \small text
\setlength\bibitemsep{0.49\baselineskip} % increase spacing between items in bibliography

% --- Make title a hyperlink to the DOI (falls back to URL)
\newbibmacro{string+doiurl}[1]{%
  \iffieldundef{doi}{%
    \iffieldundef{url}{%
      \PackageWarning{mybibliography}{Entry \thefield{entrykey} has no DOI or URL}%
      #1%
    }{%
      \href{\thefield{url}}{#1}%
    }%
  }{%
    \href{http://dx.doi.org/\thefield{doi}}{#1}%
  }%
}

\DeclareFieldFormat{title}{\usebibmacro{string+doiurl}{\mkbibemph{#1}}}
\DeclareFieldFormat[article,incollection,misc,inproceedings,book]{title}%
    {\usebibmacro{string+doiurl}{\mkbibquote{#1}}}
% ---

% --- Make biblatex hyperlinks cover the name and year instead of just year (for consistency with natbib)
\DeclareFieldFormat{citehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}% Avoid nested links
  \bibhyperref{#1}}

\DeclareFieldFormat{textcitehyperref}{%
  \DeclareFieldAlias{bibhyperref}{noformat}% Avoid nested links
  \bibhyperref{%
    #1%
    \ifbool{cbx:parens}
      {\bibcloseparen\global\boolfalse{cbx:parens}}
      {}}}

\savebibmacro{cite}
\savebibmacro{textcite}

\renewbibmacro*{cite}{%
  \printtext[citehyperref]{%
    \restorebibmacro{cite}%
    \usebibmacro{cite}}}

\renewbibmacro*{textcite}{%
  \ifboolexpr{
    ( not test {\iffieldundef{prenote}} and
      test {\ifnumequal{\value{citecount}}{1}} )
    or
    ( not test {\iffieldundef{postnote}} and
      test {\ifnumequal{\value{citecount}}{\value{citetotal}}} )
  }
    {\DeclareFieldAlias{textcitehyperref}{noformat}}
    {}%
  \printtext[textcitehyperref]{%
    \restorebibmacro{textcite}%
    \usebibmacro{textcite}}}
% ---
